MeSH Term Suggestion for Systematic Review Literature Search

High-quality medical systematic reviews require comprehensive literature searches to ensure the recommendations and outcomes are sufficiently reliable. Indeed, searching for relevant medical literature is a key phase in constructing systematic reviews and often involves domain (medical researchers) and search (information specialists) experts in developing the search queries. Queries in this context are highly complex, based on Boolean logic, include free-text terms and index terms from standardised terminologies (e.g., MeSH), and are difficult and time-consuming to build. The use of MeSH terms, in particular, has been shown to improve the quality of the search results. However, identifying the correct MeSH terms to include in a query is difficult: information experts are often unfamiliar with the MeSH database and unsure about the appropriateness of MeSH terms for a query. Naturally, the full value of the MeSH terminology is often not fully exploited. This paper investigates methods to suggest MeSH terms based on an initial Boolean query that includes only free-text terms. These methods promise to automatically identify highly effective MeSH terms for inclusion in a systematic review query. Our study contributes an empirical evaluation of several MeSH term suggestion methods. We perform an extensive analysis of the retrieval, ranking, and refinement of MeSH term suggestions for each method and how these suggestions impact the effectiveness of Boolean queries.

==> relatedwork.tex <==
\section{Related Work}


%Because of the limitations of the PubMed ATM, many works are done to optimise the ATM process. Thirion et al.~\cite{adlassnig2009optimization} proposed a method to optimise the ATM process by constructing the same search query including the mapped MeSH term and all synonyms for any user search which includes either MeSH terms or synonyms under the assumption that the same concept is sought for by the users no matter they entered a MeSH term or a synonym. Although their proposed optimisation method improved the search effectiveness by increasing the precision (might be biased since assessment is based on title and abstract only), this optimisation is not applied when the initial term is not mapped with the MeSH Translation Table under ATM, hence the optimisation process is depending on successful mappings of ATM. Massonnaud et al.~\cite{massonnaud2019performance} proposed another alternative optimisation of the PubMed query, which generates synonyms from CISMeF mappings to expand end-user query. This optimisation method is similar with the one proposed by Thirion, they both aimed to expand the user query to include MeSH terms as well as all synonyms through different mapping techniques, they both can increase the overall precision but still depending on whether the ATM mapping is successful or not, this optimisation will not be applied if the initial term cannot be mapped to MeSH Terms with ATM process.

\cite{lu2009evaluation} evaluate ATM as a way of query expansion for TREC genomics track

\cite{lu2009finding}: suggestion  of query terms in PubMed. This is for natural language terms, not MeSH.

\cite{smith2004examination} some  analysis of PubMed Automatic Term Mapping (ATM)\footnote{\url{https://www.nlm.nih.gov/bsd/disted/pubmedtutorial/020_040.html}}.

\todo{[this is just for us, not to be used as it's copy and  paste:]``Alternatively, PubMed employs a process called Automatic Term Mapping (ATM) that compares and maps untagged terms from the user query to lists of pre-indexed terms in PubMed’s translation tables (in this order): the Medical Subject Headings (MeSH) table (mapping search terms to MeSH concepts), the journals translation table (mapping search terms to journal names), and the author index (mapping search terms to author names). By default, PubMed applies the Automatic Term Mapping feature to every unqualified user query, thus affecting the search results of millions of user queries each day in spite of the fact that many users may not actually realize its existence. It is designed and implemented by the NLM as a means to improve retrieval performance. ''}
	
\cite{nahin2003change} explains how ATM works. (note, may be  old).

\cite{adlassnig2009optimization} attempts to optimise ATM.

\cite{massonnaud2019performance} expands MeSH portions of queries with other semantic resources.

\cite{richter2012using}: have a read. May provide use case, and also queries.


provision of use case/motivation:  \cite{chang2006searching}: \todo{ ``Two search strategies, one based on the use of Medical Subject Headings (MeSH) and the second based on text word searching, were compared.  The MeSH search provided a more efficient search than the text word search.}


Motivation: \cite{liu2017evaluating} ``The usefulness of controlled vocabularies, exemplified by Medical Subject Headings (MeSH), was evaluated by a controlled user experiment. MeSH terms were most useful for domain experts in terms of precision measure.''


\cite{zieman1997conceptual}: \todo{`` describes a way to map users' queries to relevant Medical Subject Headings (MeSH terms) used by the National Library of Medicine to index the biomedical literature''}  from 1997


\cite{liu2009impact} phd thesis focused  on effectiveness of MeSH for search.

==> search_effectiveness.tex <==




==> table_seperate.tex <==


